Cuttlefish: Expressive Fast Path Blockchains with FastUnlock

Cuttlefish addresses several limitations of existing consensus-less and consensus-minimized decentralized ledgers, including restricted programmability and the risk of deadlocked assets. The key insight of Cuttlefish is that consensus in blockchains is necessary due to contention, rather than multiple owners of an asset as suggested by prior work. Previous proposals proactively use consensus to prevent contention from blocking assets, taking a pessimistic approach. In contrast, Cuttlefish introduces collective objects and multi-owner transactions that can offer most of the functionality of classic blockchains when objects transacted on are not under contention. Additionally, in case of contention, Cuttlefish proposes a novel `Unlock' protocol that significantly reduces the latency of unblocking contented objects. By leveraging these features, Cuttlefish implements consensus-less protocols for a broader range of transactions, including asset swaps and multi-signature transactions, which were previously believed to require consensus.

==> sections/crdts.tex <==

\section{Leveraging Commutativity for Maximum Parallelism}
\lef{The formalization and exploration of this together with applications can be the project of an intern}

When applying commutative operations on an object, we could avoid any risk of locking if an appropriate commutative data-structure is implemented.
Unfortunately, in a practical system where gas needs to be paid no transaction can have only fully commutative operations as substraction with comparison to zero is not a monotonic operation~\cite{xxx}. This, nevertheless, is a problem that would appear only if the client does bad accounting on their side. Additionally, the fast-unlock protocol gives us the ability to recover when this happens. Thanks to these observation we manage to enhance our programmability with commutative and mostly-commutative objects.

Mostly-commutative objects admit commutative operation most of the time and define an invariant that if locally violated safety is at risk. For example payments are usually commutative until the account has no more money.
Then, we let operations run in parallel but compare every write with an invariant (is there more budget to spend?). When the invariant is locally violated the validator will block the fast path. As a result, when f+1 honest validators block their fast path we know that we are at risk of a global safety violation. Using the fast-unlock workflow we can consolidate all valid transactions and arrive at a consistent state.

In this section we provide multiples implementations of data structures that leverage commutativity
in order to extract maximum parallelism out of a workload. More specifically we show how to implement an commutative counters and sets as well as a mostly-commutative bounded-counter. We then show how to implement the most popular types of smart-contracts using these data-structures as well as multi-agent transaction.


\subsection{Commutative Counters}

Implementing a counter/account that only receives credit transactions is easy as there is no risk of unsafe operations. The design is inspired by G-counters from CRDTs~\cite{xxx}. Since we need to provide auditability of all updates we opt for an update based G-counter. The protocol works as follows:


\begin{enumerate}
    \item The client prepares a credit transaction for the account and sends it to the validators using the same workflow as a transaction.
    \item The validators check the objects that are to be consumed and lock-them as usual; any object that is tagged as commutative is not locked but we still need to check that it exists (Algortihm~\ref{alg:process-crdt-cert})~\Cref{alg:line:process-cert-load-comm-objects}). \lef{abusing the fact that this should happen both in processtx and process cert}
    \item The client generates a lock-certificate as before and sends it to the validators.
    \item The validators process the lock-certificate. In principle the only difference from classic exectuion is that the
          commutative objects do not have a specific new version number (\Cref{alg:line:execute-cert}), but are simple marked as ''credit-accepted''. As before, the validator also sends the transactions to be checkpointed after veryfying the certificate (\Cref{alg:line:forward-to-checkpoint}).
\end{enumerate}

\begin{algorithm}[t]
    \caption{Process certificate with commutative objects}
    \label{alg:process-crdt-cert}
    \small
    \begin{algorithmic}[1]
        \Require Input certificate \Cert is signed by a quorum
        \Statex
        \Statex // Executed upon receiving a certificate from a user.
        \Statex // Many tasks can call this function.
        \Procedure{ProcessCert}{$\Cert$}
        \State // All valid certificates are checkpointed.
        \State \Call{ForwardToCheckpoint}{$\Cert$} \label{alg:line:forward-to-checkpoint}
        \State // Load owned objects from store, return error if missing.
        \State $[\Obj_{o}] \gets \Call{LoadObjects}{\txinputs{\Cert}}$ \label{alg:line:process-cert-load-owned-objects}
        \State // Check commutative objects exist, return error if missing.
        \State $\Call{CheckObjects}{\txcommutativeinputs{\Cert}}$ \label{alg:line:process-cert-load-comm-objects}
        \State
        \State // Check the owned objects locks.
        \If{\Call{LocksExist}{$\Cert$}} \label{alg:line:ensure-locks-exist}
        \State // Execute the certificate. \label{alg:line:execute-cert}
        \State $\effectvote, [\Obj_{out}], [\Obj_{com}] \gets \exec{\Cert, [\Obj_{o}]}$ \label{alg:line:exec}
        \State \Call{AtomicPersist}{$\Cert, \effectvote, [\Obj_{out}], [\Obj_{com}]$}  \label{alg:line:atomic-persist}
        \State \Return \effectvote
        \EndIf
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

Using the same algorithm we can make a commutative counter that allows for both additions and subtractions. The canonical way to achieve this is to have two G-counter one for additions and one for subtractions, however in our case we can simply allow validators to admit both additions and subtractions to the counter and consolidate all updates at consensus when we need to read the counter.

\subsection{Commutative Sets}

Similar to a G-Counter we can create a Union Set (U-Set) that allows to only add items in the set. The workflow is the same as the G-Counter. As long as f+1 honest parties remember that an item is added in the Set we have a guarantee that it will not be forgotten in a checkpoint.
This approach can be generalized to any monotonic program~\cite{calm}. For example we can create a PN-Set by using two U-sets one for adding items and one for adding tombstones. The PN-Set is all the items of the additions set that are not part of the tombstones set.

\subsection{Bounded Counter} \lef{TODO: Formal proofs}
Although commutative data structures can enable significant parallelism in \sys they only work for monotonic programs
However, we cannot provide any guarantees that the PN-counter will not have a negative balance, since an 'if-close' breaks monotonicity, making this an unsuitable data-structure for representing account balances. Instead we need to implement a Bounded Counter~\cite{shapiro}.
There currently exists a single protocol that implements a concurrent bounded counter and it only works if all validators/replicas are honest and do not crash.
The basic idea is that every validator gets a separate budget from the total value of the counter which is allowed to be spent concurrently. If this reaches zero then validators can transfer budget between each other.

This approach unfortunately cannot be directly used in our setting for two reasons. First, nodes can crash, meaning that part of the budget might never be used as we cannot differentiate between a crashed and a slow but correct party in asycnhrony. Second, nodes can lie, meaning that we cannot allow transfers between nodes like prior work. Instead we design \textit{the first BFT Bounded counter which admits concurrent substractions}.
To this end, we  reuse the idea of having a budget in the counter and leverage the  existence of the Fast-Unlock protocol.
Our bounded counter allows for concurrent substraction up to $50\%$ of the maximum bound.
When this is reached, validators will block the concurrent path forcing the client to fall-back to consensus and generate a new bounded counter with a new lower budget which is once again half of the outstanding credits; as a result with only log(MaxCredit) consensus executions we can spend the full value safely and concurrently.



\begin{enumerate}
    \item The client prepares a transaction for the account and sends it to the validators.
    \item The validators check the objects that are to be consumed and lock-them as usual, they also check that the account to be credited is tagged as Bcounter.If the transactions is a credit transaction they do not need to lock anything. If the transaction is a debit transaction they try to substract atomically the value from the \emph{Budget}. If the outstanding Budget is positive they return a lock. Otherwise they add back the value and reject the transaction.
    \item The client generates a lock-certificate as before and sends it to the validators.
    \item The validators produce an execution state where the account to be credited does not have a specific new version number, but it is simple marked as ''transaction-accepted''. If the transaction was a credit transacation they increase the budget atomically by $\frac{credit}{2}$.
\end{enumerate}



\begin{algorithm}[t]
    \caption{Process transaction with bounded counter}
    \label{alg:process-tx-bc}
    \small
    \begin{algorithmic}[1]
        \Require Input certificate (\tx) is signed by a client
        \Statex
        \Statex // Executed upon receiving a transaction from a user.
        \Statex // Many tasks can call this function.
        \Procedure{ProcessTx}{$\tx$}
        \State // Load owned objects from store, return error if missing.
        \State $[\Obj_{o}] \gets \Call{LoadObjects}{\tx}$ \label{alg:line:process-tx-load-owned-objects}
        \State // Load commutative objects, only BC counter return.
        \State $[\Obj_{bc}] \gets \Call{CheckObjects}{\tx}$ \label{alg:line:process-tx-load-comm-objects}
        \State
        \State // Lock owned objects, reject if it fails
        \For{$\Obj \in [\Obj_{o}]$}
        \If{!\Call{Lock}{$\Obj$}}
        \Return
        \EndIf
        \EndFor
        \State // Substract Bounded Counter Value and check> 0. \label{alg:line:execute-cert}
        \For{$\Obj \in [\Obj_{bc}]$}
        \If{!\Call{Substract}{$\Obj.budget, \tx$}}
        \Return
        \EndIf
        \EndFor
        \State \Return \lockvote
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \caption{Process certificate with bounded counter}
    \label{alg:process-bc-cert}
    \small
    \begin{algorithmic}[1]
        \Require Input certificate (\Cert) is signed by a quorum
        \Statex
        \Statex // Executed upon receiving a certificate from a user.
        \Statex // Many tasks can call this function.
        \Procedure{ProcessCert}{$\Cert$}
        \State  // All valid certificates are checkpointed
        \State \Call{ForwardToCheckpoint}{$\Cert$} \label{alg:line:forward-to-checkpoint}
        \State // Load owned objects from store, return error if missing.
        \State [$\Obj_{o}$] = \Call{LoadObjects}{$\txinputs{\Cert}$} \label{alg:line:process-cert-load-owned-objects}
        \State // Check commutative objects exist, return error if missing.
        \State \Call{CheckObjects}{$\txcommutativeinputs{\Cert}$} \label{alg:line:process-cert-load-comm-objects}
        \State
        \State // Check the owned objects locks.
        \If{\Call{LocksExist}{$\Cert$}} \label{alg:line:ensure-locks-exist}
        \State // Execute the certificate. \label{alg:line:execute-cert}
        \State $\effectvote, [\Obj_{out}], [\Obj_{com}] = \exec{\Cert, [\Obj_{o}]}$ \label{alg:line:exec}
        \State
        \State // For credits atomic increment budget
        \For{$\Obj \in [\Obj_{com}]$}
        \If{$\Obj$.type= bc}
        \Call{CreditHalf}{$\Obj.budget, \tx$}
        \EndIf
        \EndFor
        \State
        \State \Call{AtomicPersist}{$\Cert, \effectvote, [\Obj_{out}], [\Obj_{com}]$}  \label{alg:line:atomic-persist}
        \State \Return \effectvote
        \EndIf
        \EndProcedure
    \end{algorithmic}
\end{algorithm}


At some point the Budget of f+1 honest parties will be $0$, then the concurrent path can no longer be used. Instead any authorized party can request a fast-unlock of the Bcounter. At the fast-unlock step parties return the set of transactions they have seen a certificate but are not checkpointed in the consensus. The driving party collects 2f+1 replies and submits them to consensus for consolidation (similar to~\cref{sec:multi-unlock}). When all transactions have been executed there is a new Bounded counter with a new MaxCredit. The valdiators then set their budget to $\frac{MaxCredit}{2}$ and re-enable the concurrent path. Any transactions trying to touch the old B-Counter will no longer be valid since the version of the counter will be updated.

\begin{theorem}[Bounded Counter Safety] \label{th:unlock-liveness}
    The global credit value does not get negative
\end{theorem}

\begin{proof}
    The counter has a value MaxCredit of the of credits allowed to be spent. We assign every validator $\frac{MaxCredit*(f+1)}{2f+1}$ budget.
    \alberto{Didn't we say we assign a budget of $\frac{MaxCredit}{2}$ to each validator?} \lef{help with the proof and is approximately half}
    Hence in an honest concurrent execution at most $\frac{MaxCredit}{2}$ can be spent. Now we show that the adversary cannot use its equivocation power (i.e., infinite budget for f parties) to spend more than  MaxCredit. Taking a unit-valued transaction, in order for it to be valid it need $2f+1$ approvals, out of which $f+1$ are honest. Hence from the total amount of credit that honest parties have there needs to be $f+1$ budget reduced. But there is only MaxCredit*(f+1) budget assigned collectively to all honest parties. As a result there can only be at most MaxCredit spend in the concurrent path.
\end{proof}






%A natural question here, is what happens when the user wants to consolidate such a commutative object to a deterministic value, that e.g., serves as an input to a more complex smart contract. 
%Then the fast-unlock procedure can be used to block the object's processing and consensus can be used to do the consolidation. The checkpoint mechanism currently used in Sui is nothing more than a simple use-case of this workflow. The fast path of Sui only admits per-object operations, which are by definition commutative when applied to the global state. So if we see the full state as a single object the during reconfiguration
%what happens is that processing on the fast path is blocked (can be also done through the fast-unlock workflow) and consensus consolidates the sate towards a consistent checkpoint.



%Notice that the add-only counter will never fail and as a result does not really need to lock objects, it could skip the lock-phase of Sui and return and execution certificate in one RTT.  However, this is only true for data-structures that do not have an assert clause every time they are updated.  Given that all transactions need a gas object, which might at some point be depleted of gas, this observation is impractical for \sys. Hence, all transactions follow the classic lock-then-execute workflow of Sui and can leverage the Fast-Unlock either to produce a consistent read or to unblock because a mostly-commutative object was under contention that woudl result in an illegal state if not blocked. 




==> sections/implementation.tex <==

\section {Evaluation}


\subsection{Applications of \sys}

Now that we have discussed how to allow for more than owned objects without consensus,
we discuss how the most popular blockchains applications can leverage this to maximize efficiency.


\paragraph{StableCoins/Multi-sig wallets}

\lef{evaluate an application on \sys for stable coins or 1-out-of-2 multisig}

\paragraph{Atomic swaps}

\lef{evaluate an application of \sys on concurrent atomic swaps on objects that are not under contention}

\paragraph{Batching consensusless transactions to increase throughput}
\lef{evaluate different batch sized of owned objects transactions to show tha latency/throughput tradeoff. This serves as an application from a DApp developers (e.g., game) that does not want to pay 1 certificates per object accesed}


% \paragraph{Peer-to-Peer Transfers and ERC-20 Tokens}
% The initial reason blockchain protocols were designed and the most popular one is to simply transfer value between to peer parties.
% This application has severe issues when hot-accounts are used to receive value, as they are currently a point of serialization.
% Using a G-counter we can instead persist credit transactions to hot accounts in parallel as addition is a commutative operation.
% Furthermore, we can leverage bounded-counters in case the debit account is also under contention to achieve fully parallelizable P2P transfers.

% Similar to P2P transfers we can also parallelized ERC-20 Tokens, one of the most used smart-contracts for token creations, especially stable-coins.
% As far as commutative is concerned we need the same data-structures with the extra requirement that these transactions might need authorization from a regulator or the smart-contract creator. The additional functionality is provided by multi-agent transactions described in Section~\ref{sec:xxx} and any chance of locking due to contention can easily be resolved by invoking the fast-unlock protocol of Section~\ref{sec:xxx}.

% \lef{Evaluation of p2p transfers where the recipient is the same address (e.g., a popular merchant or content creator)}

% \paragraph{NFT Creation and Trading}
% On Ethereum NFTs usually follow the
% EIP-721 Standard and most NFT standards across the
% industry derive from this initial standard. There are two data
% structures related to the creation(minting) of NFTs in this
% standard:
% \begin{itemize}
%     \item Mapping from token ID to owner address
%     \item Mapping from user address to approved address mapping to count
% \end{itemize}
% Typically, during the process of creating a new NFT (called minting), a counter is incremented which returns the unique IDof the NFT. Based on this ID, the NFT is then connected with the new owner address (the user invoking the smart contract) by inserting them into the respective mapping. In order to implement NFT Creation using our commutative data-structures we need a bounded-counter and a U-Set. The parties can then decrement by one the bounded counter and simultaneously add themselves in the map. Later, during consolidation they counter will result in a unique-ID for the NFT.

% For NFT Trading, there is the additional need to remove a party from set of owners once the item is sold. As a result enhancing the workflow with a PN-Set should be sufficient.
% \deepak{This might be restrictive. My understanding of a PN-set is that once an element is removed, it can never be re-added, i.e., you can only own an NFT once.} 
% \lef{This is true, basically you cannot buy with the same pseudonym, but you can randomize your pseudonym to buy again in order to circumvent the issue}

% \lef{evaluate an application of \sys on an NFT public-sale of a limited number of assets}

%\paragraph{Dexes and AMMs}
%ne final important application of blockchain is Decentralized Exchanges. These can be implemented with two different architectures.
%The first architecture is a decentralized order-book. We can increase the concurrency of the order book by implementing it with a U-Set. Parties can independently put their orders without having to wait each other.
%The periodically the order-book will go through consensus to match orders and garbage collect the part of the U-set that is traded successfully.
%An AMM can also be implemented concurrently if we sacrifice dynamic price adjustment between consensus invocations. If the price of trade is fixed the AMM can use bounded counters to trade all assets without risking overdraft.



%\george{This is high-value: I think we can define an update tx output sent to an object, with different updated being applied async from each other to the object. But once the object is included in a tx (for read) all must have a consistent view. Does that work?} 
%\lef{Yes we can define "write-only" objects for the fast path that are read only by consensus. Then we can define write-only with assert objects that run an assertion on every right to see if the local invariant holds. I will explore further litrature}

\subsection{Evaluate \fun}
\lef{Evaluate how fast we can regain liveness with an increasing number of validators}
\lef{Evaluate how much better throughput we can do by batching transactions from different sources, this risks liveness if there is contention but it is highly unlikely}

\subsection{Implementation} \label{sec:implementation}
\alberto{TODO: describe how to make \cref{alg:process-unlock-tx}, \cref{alg:process-unlock-cert}, \cref{alg:process-unlock-tx-multi}, and \cref{alg:process-unlock-cert-multi} thread-safe (also with respect to the other algorithms).}



==> sections/multi-unlock-algo.tex <==
\section{Multi-Object Unlock Protocol} \label{sec:multi-unlock-algorithms}
This section details the algorithms run by the \sys validators when running the multi-object unlock protocol described in \Cref{sec:multi-unlock}.
%
Validators respectively run \Cref{alg:process-unlock-tx-multi} and \Cref{alg:process-unlock-cert-multi} when receiving an unlock request $\unlockreq$ and unlock certificate $\unlockcert$ over multiple objects.

\noindent
\scalebox{0.75}{
    \noindent
    \begin{minipage}[t]{0.62\textwidth}
        \input{algorithms/process-unlock-tx-multi}
    \end{minipage}
    \hskip 0.5em
    \begin{minipage}[t]{0.68\textwidth}
        \input{algorithms/process-unlock-cert-multi}
    \end{minipage}
}




% \begin{algorithm}[t]
%     \caption{Process unlock messages}
%     \label{alg:process-unlock-tx-multi}
%     \footnotesize
%     \begin{algorithmic}[1]
%         \Statex // Handle $\unlockreq$ messages from clients.
%         \Procedure{ProcessUnlocktTx}{$\unlockreq$}
%         \State // Check (\ref{alg:process-unlock-tx-multi}.1): Check authenticator.
%         \If{$!\valid{\unlockreq}$} \Return error \EndIf \label{alg:line:check-abort-multi}

%         \State
%         \State // Collect certificates.
%         \State $c \gets \none$
%         \For{$\Okey \in \unlockreq.\Okeys$}
%         \State $c \gets c \cup \lockdb[\Okey]$ \label{alg:line:check-cert-multi}
%         \EndFor
%         \State $\unlockvote \gets \sign{\unlockreq, c}$

%         \State
%         \State // Record the decision to unlock.
%         \If {$c==\none$}
%         \For{$\Okey \in \unlockreq.\Okeys$}
%         \State $\unlockdb[\Okey] \gets \unlocked$ \label{alg:line:block-exec-multi}
%         \EndFor
%         \State
%         \EndIf
%         \State \Return $\unlockvote$
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[t]
%     \caption{Process unlock certificates}
%     \label{alg:process-unlock-cert-multi}
%     \footnotesize
%     \begin{algorithmic}[1]
%         \Statex // Handle $\unlockcert$ messages from consensus.
%         \Procedure{ProcessUnlockCert}{$\unlockcert$}
%         \State // Check (\ref{alg:process-unlock-cert-multi}.1): Check message validity.
%         \For{$\Okey \in \unlockcert.\Okeys$}
%         \If{$\unlockdb[\Okey] = \confirmed$} \Return \EndIf \label{alg:line:ensure-first-multi}
%         \EndFor

%         \State
%         \State // Check (\ref{alg:process-unlock-cert-multi}.2): Check message validity.
%         \If{$!\valid{\unlockcert}$} \Return error \EndIf \label{alg:line:check-abort-multi-cert}

%         \State
%         \State // Check (\ref{alg:process-unlock-cert-multi}.3): Can we execute the tx?
%         \State $v \gets [\;]$
%         \If{\unlockcert.\cert = [\;]}  \label{alg:line:no-overwrite-multi}
%         \State $\tx \gets \unlockcert.\unlockreq.\tx$
%         \State $\effectvote \gets \exec{\tx, \unlockcert}$ \label{alg:line:exec-tx-multi}
%         \State $v \gets \effectvote$
%         \For{$\Okey \in \unlockcert.\Okeys$}
%         \State $\unlockdb[\Okey] = \confirmed$
%         \EndFor
%         \Else
%         \For{$\Cert \in \unlockcert.\cert$}
%         \State $\effectvote \gets \exec{\Cert}$ \label{alg:line:exec-multi}
%         \State $v \gets v \cup \effectvote$
%         \For{$\Okey \in \cert.\Okeys$}
%         \State $\unlockdb[\Okey] = \confirmed$ \label{alg:line:mark-confirmed-multi} %not really necessary since checkpoints will eventually do the same
%         \EndFor
%         \EndFor
%         \EndIf

%         \State \Return $v$
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

